DeReStainer: H&E to IHC Pathological Image Translation via Decoupled Staining Channels

Breast cancer is a highly fatal disease among cancers in women, and early detection is crucial for treatment. HER2 status, a valuable diagnostic marker based on Immunohistochemistry (IHC) staining, is instrumental in determining breast cancer status. The high cost of IHC staining and the ubiquity of Hematoxylin and Eosin (H&E) staining make the conversion from H&E to IHC staining essential. In this article, we propose a destain-restain framework for converting H&E staining to IHC staining, leveraging the characteristic that H&E staining and IHC staining of the same tissue sections share the Hematoxylin channel. We further design loss functions specifically for Hematoxylin and Diaminobenzidin (DAB) channels to generate IHC images exploiting insights from separated staining channels. Beyond the benchmark metrics on BCI contest, we have developed semantic information metrics for the HER2 level. The experimental results demonstrated that our method outperforms previous open-sourced methods in terms of image intrinsic property and semantic information.

==> parts/Method496.tex <==
\section{Methods} %字大点
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/modelfiglaji.png}
    % \caption{The overall architecture of our framework. H\&E images are inputted into the DeStainer to remove the E channel and subsequently brought closer to the H channel of IHC images in the high-dimensional feature space. The high-level representation of $I_{H\&E}^H$ and the level information of HER2 are directed into the feature fusion module and the Restainer generates the corresponding IHC images. In the framework, y is the HER2-level label of input IHC image $f$ represents a simple network, C and D are comparator and discriminator respectively.  }
    \caption{The overall architecture of our framework. DeStainer performs stain separation and aligns the H channel of H\&E with that of IHC images. The Feature Fusion Module integrates the output of DeStainer with the classification information of the HER2 level. Restainer is used to generate the corresponding IHC images. In the framework, y is the HER2-level label of the input IHC. $f$ represents a simple network, C and D are comparator and discriminator respectively. }
    \label{model}
\end{figure}

% In practical medical pathological staining, both H\&E and IHC staining use hematoxylin as a dye to make the structure of the cell nucleus more prominent. Consequently, we propose DeReStainer, a framework for automatic translation from H\&E to IHC images. 
As is shown in \autoref{model}, our proposed DeReStainer mainly contains a DeStainer and a ReStainer. The DeStainer aligns the H channel that is shared between H\&E and IHC images, while the ReStainer is responsible for applying DAB staining to generate the corresponding IHC images. 
% H通道什么的搞成上标，不要下标
Without further notice, we denote the H\&E image, generated IHC image, and the ground truth IHC image as $I_{H\&E}, \hat{I}_{IHC}, I_{IHC}$ respectively. 

\subsection{DeStainer}
The DeStainer aims to embed the H channel of both H\&E and IHC images into a high-dimensional feature space and align them with each other.
%%得引入下，不能直接硬
To get the H channel from the corresponding H\&E and IHC images, these images are first sent to the staining separation module in the DeStainer. The staining separation module uses a staining separation algorithm based on color space transform \cite{ruifrok2001quantification} to separate input pathology images into the H channel and the other channels (E channel for H\&E and DAB channel for IHC image). Specifically, it first maps a tissue pathology image in the RGB space to the HED (Hematoxylin, Eosin, DAB) space. A projection matrix is then applied to map the image in HED space to a certain channel by setting the other two channels of this image to zero. After that, the resulting image is transformed back to RGB space to get the separated channel result. 
% For instance, if we want to get the H channel of an H\&E image, the procedure is shown in the following formula, in which the $P$ represents the HED space transformation matrix, and $P^{\dagger}$ is its inverse. The same procedure will be performed on $I_{IHC}$ to get $I_{IHC}^H$ and for the $I_{IHC}^{DAB}$, the H and E channels will be eliminated instead. 
 For instance, the procedure to get the H channel of an H\&E image is shown in the following formula, where
%  $ \begin{bmatrix}
% v_H & v_E & v_{DAB} 
% \end{bmatrix}
%  = P\cdot I_{H\&E}^{RGB} $, and we eliminate the E and DAB channel, which are $v_E, v_{DAB}$ and finally transform the result back to RGB space to get $I_{H\&E}^H = 
% \begin{bmatrix}
% v_H & \bar{0} & \bar{0} 
% \end{bmatrix}
%  \cdot P^{\dagger}$. 
 $T(\cdot):\mathbb{R}^{n\times n\times 3} \rightarrow \mathbb{R}^{n\times n\times 3}$ is the transform from RGB to HED space, $P^H \in \text{M}_3(\mathbb{R})$ represents projection matrix to H channel. 
$$
\begin{aligned}
& I_{H\&E}^{HED}= \left[v_H, v_E, v_{DAB}\right]=T(\left[v_R, v_G, v_B\right])=T(I_{H\&E}^{R G B}) \\ 
& I_{H\&E}^H=\left[v_R^{\prime} , v_G^{\prime}, v_B^{\prime}\right]=T^{-1}(\left[v_H, 0,0\right]) =T^{-1}(\left[v_H , v_E, v_{DAB}\right] \cdot P^H) 
\end{aligned}
$$
We perform the same procedure on $I_{IHC}$ to get $I_{IHC}^H$. For the separation of $I_{IHC}^{DAB}$ from $I_{IHC}$, we use $P^{DAB}\in \text{M}_3(\mathbb{R}) $ as the projection matrix thus the DAB channel is retained instead.

% \begin{equation*}
%    I_{H\&E}^{RGB}\xrightarrow{P} I_{H\&E}^{HED}=\begin{bmatrix}
% | & | & | \\
% v_H & v_E & v_{DAB} \\
% | & | & |
% \end{bmatrix} \xrightarrow{v_E,v_{DAB}=\bar{0}} \begin{bmatrix}
% | & | & | \\
% v_H & \bar{0} & \bar{0} \\
% | & | & |
% \end{bmatrix} \xrightarrow{P^{\dagger}} I_{H\&E}^{RGB'}=I_{H\&E}^H
% \end{equation*}
% \begin{equation*}
%     I_{H\&E}^H = P \cdot  I_{H\&E}^{RGB} \cdot 
% % \begin{bmatrix}
% % 1 & 0 & 0 \\
% % 0 & 0 & 0 \\
% % 0 & 0 & 0
% % \end{bmatrix} 
% Q
% \cdot P^{\dagger} %= I_{H\&E}^{HED} \cdot Q(1)
% %     \begin{bmatrix}
% % 1 & 0 & 0 \\
% % 0 & 0 & 0 \\
% % 0 & 0 & 0
% % \end{bmatrix} 
% %\cdot P^{\dagger} 
% = 
% \begin{bmatrix}
% v_H & v_E & v_{DAB} 
% \end{bmatrix} \cdot Q
% % \begin{bmatrix}
% % 1 & 0 & 0 \\
% % 0 & 0 & 0 \\
% % 0 & 0 & 0
% % \end{bmatrix} 
% \cdot P^{\dagger} = \begin{bmatrix}
% v_H & \overset{\bar{0}}{\cancel{v_{E}}}  & \overset{\bar{0}}{\cancel{v_{DAB}}} 
% \end{bmatrix} \cdot P^{\dagger}  
% \end{equation*}
% We denoted the image we want to process as $I$. The stain separation result can be formulated as
% $I_{result}= \exp{((\log I) PQP^{\dagger})}$.
% The $P$ is the projection matrix to HED space, $P^{\dagger}$ is its pesudo inverse and $Q$ is channel elimination matrix, which is defined as
% \[
% % P = \begin{bmatrix}
% % 0.65 & 0.70 & 0.29 \\
% % 0.07 & 0.99 & 0.11 \\
% % 0.27 & 0.57 & 0.78
% % \end{bmatrix} \quad
% \[
% Q(c) = \begin{bmatrix}
% \delta(1, c) & 0 & 0 \\
% 0 & \delta(2, c) & 0 \\
% 0 & 0 & \delta(3, c)
% \end{bmatrix} \quad
% \delta(i, c) = \begin{cases} 
% 1, & \text{if } i = c\in\{1,2,3\} \\
% 0, & \text{otherwise}
% \end{cases}
% \]
% where $\delta(i, c)$ be a function defined as
% \[
% \delta(i, c) = \begin{cases} 
% 1, & \text{if } i = c \\
% 0, & \text{otherwise}
% \end{cases}
% \]
% where $i\in \{1, 2, 3\}$ corresponds to the matrix index and $c \in \{1, 2, 3\}$ corresponds to the channel we wish to retain (1 for H, 2 for E, 3 for DAB). The values in the matrix that contain the information of the others two channels are set to 0.
%encoder的E字母要换了，用f这种，介绍符号的往上，最后那个align要另起一段清楚些
% \begin{equation*}
%  [v_H,  v_E,  v_{DAB} ]
%  = P\cdot I_{H\&E}^{RGB},
% I_{H\&E}^H = 
% [v_H, \bar{0}, \bar{0}]
%  \cdot P^{\dagger}   
% \end{equation*}
$I_{H\&E}^H$ and $I_{IHC}^H$ from the staining separation module are sent into the encoder of DeStainer to get their the high-level representations. After that, these high-level representations are sent into $f_{H}$ to be aligned with each other. We designed $L_{{H}}$ to constrain this process, which is a cosine similarity loss defined as:
\begin{equation}
L_{{H}} = 1-\frac{\langle f_{H}(\text{DeStainer}(I_{H\&E}^H), f_{H}(\text{DeStainer}(I_{IHC}^H))\rangle}{|f_{H}(\text{DeStainer}(I_{H\&E}^H)|\cdot|f_{H}(\text{DeStainer}(I_{IHC}^H))|}
\end{equation}
% Additionally, $DeStainer(I_{H\&E,H})$ is directed into $E_{level}$, which concludes with a linear layer for the prediction of HER2 level, utilizing focal loss \cite{lin2017focal} as the loss function. The classification information encoded by $E_{level}$, along with the Hematoxylin channel features of the H\&E images encoded by the DeStainer, are jointly directed into the Feature Fusion module.

\subsection{Feature Fusion Module}
The feature fusion module aims to combine the feature of $I_{H\&E}^H$ and the HER2 level information to help generate IHC images with precise HER2 level. 

Before being sent into the feature fusion module, the high-level feature of $I_{H\&E}^H$ is directed to $f_{H}$ to get classification information for HER2 level, denoted as $\hat{S}_{HER2}$. Then, $\hat{S}_{HER2}$ will sent jointly with the output of DeStainer to the feature fusion model to get the input of ReStainer. It is modified from typical ResNet blocks and the convolutional layer in it is modified to modulation convolutional block in StyleGAN2 \cite{stylegan}, which performs weight demodulation operation.
The demodulation operation of modulation convolutional block can be formulated as
\begin{equation}
   \text{ModConv}(x,\hat{S}_{HER2}) = \text{Conv}\left( x, \frac{W \times (\hat{S}_{HER2} + 1)}{\sqrt{\sum(W \times (\hat{S}_{HER2} + 1))^2 + \epsilon}} \right) + b , 
\end{equation}
where $\texttt{Conv}$ is 2-d convolution, $W$ is the original weight of the convolutional layer, $b$ is an optional bias, and $\epsilon$ is a small constant.
Beyond that, SimAM \cite{simam}, a parameter-free attention layer is appended on the end of each block. 
% Denote the input of a basic block as $x$, the classification information from $E_{level}$ as $\hat{S_{HER2}}$, then the output of each block can be formulated as
% $$
% y = Att(ActMod^2(x,\hat{S_{HER2}}))+x
% $$
% In which $Att$ is the SimAM\cite{simam}, a parameter-free attention layer. $ActMod$ is the composition of an activation function and a weight demodulation operation. 



\subsection{ReStainer}
The ReStainer is a decoder that is symmetric to the encoder of the DeStainer. The goal is to apply DAB staining on the output of the feature fusion module to generate the corresponding IHC images. We employ a staining separation module identical to that in the DeStainer to obtain $\hat{I}_{IHC}^{DAB}$ and $I_{IHC}^{DAB}$. To further improve staining quality, we have formulated 
$ L_{{DAB}}$, which is defined as:
\begin{equation}
L_{{DAB}} = \|\hat{I}_{IHC}^{DAB}-I_{IHC}^{DAB}\|_1
\end{equation}
Beyond the ReStainer, we incorporate a comparator and a discriminator into our framework. The comparator aims to bring the generated IHC images closer to real IHC images on the feature level, further strengthening the control of visual perception. The discriminator applies generative adversarial learning to make the generated IHC images more realistic. 
% \subsection{Loss Functions}
% % In our framework, several loss functions were applied to constrain the image content as well as the semantic information of the generated IHC image. This section describes the losses including content loss, semantic loss, GAN loss and Detaining loss in detail.
% % This section summarizes the loss functions used in our framework, which contains stain loss and other auxiliary loss including content loss, semantic loss, and GAN loss.

% % Apart from the staining loss aimed to control the destain and restain steps separately through the loss constructed from the separated H and DAB channels, which can be formulated as $
% % L_{Stain} = \lambda_{H}L_{H}+\lambda_{DAB}L_{DAB}
% % $, there are other auxiliary loss including content loss, semantic loss, and GAN loss in our framework.
% % \subsubsection{Stain Loss}
% % The Staining loss is a loss function proposed in conjunction with a stain separation algorithm, designed to regulate the effects of de-staining and re-staining. This loss function comprises two components: Hematoxylin loss \( L_{\text{Hematoxylin}} \) and DAB loss \( L_{\text{DAB}} \). The Hematoxylin loss is utilized to align the high-level representations of the Hematoxylin channel in H\&E staining with the Hematoxylin channel IHC in the encoder, using a cosine similarity loss. Meanwhile, the DAB loss involves applying MAE loss to the DAB channel of both the generated IHC image and the ground truth. This approach aims to enhance the quality of the staining. The $L_{\text{Hematoxylin}}$ and $L_{\text{DAB}}$ can be formulated as 
% \textbf{Stain Loss. } The stain loss is the most significant loss in our framework, which is the weighted sum of $ L_{{H}}$ and $ L_{{DAB}}$, whose purpose and formulation have been discussed in the former section respectively. The stain loss is formulated as:
% % This section discusses the auxiliary losses presented in our framework, and all the $\lambda$s in the section represent weight constants for a certain loss function. In addition to the stain loss, the weighted sum of $L_{H},L_{DAB}$ formulated as:
% $$
% L_{stain} = \lambda_{H}L_{H}+\lambda_{DAB}L_{DAB}.
% $$
% \textbf{Auxiliary Losses. }Besides the stain loss, we also incorporates auxiliary losses, including content loss, semantic loss, and GAN loss into the framework, to facilitate the generation of IHC images.
% % Beyond the stain loss—previously detailed in an earlier section as a weighted sum of $L_{\text{H}}$ and $L_{\text{DAB}}$, and formulated by:

% % there are other auxiliary loss including content loss, semantic loss, and GAN loss in our framework.
% %and
% % % $$
% % L_{\text{Hematoxylin}} = 1-\frac{E_{hemato}(Destainer(I_{H\&E,H}))\cdot E_{hemato}(Destainer(I_{IHC,H}))}{\|E_{hemato}(Destainer(I_{H\&E,H})\| \cdot \| E_{hemato}(Destainer(I_{IHC,H})\|}, L_{\text{DAB}} = \|\hat{I_{IHC,DAB}}-I_{IHC,DAB}\|_1
% % $$
% % it can be formulated as:
% % $$
% % L_{Stain} = \lambda_{H}L_{H}+\lambda_{DAB}L_{DAB}
% % $$
% % 不要highlight其他loss

% The content loss consists of structure similarity loss \cite{ssim} $L_{ssim}$ and the mean absolute error loss $L_{mae}$. 
% % $$L_{mae} = \|\hat{IHC}-IHC\|_1,L_{ssim}=1-SSIM(\hat{IHC}-IHC)
% % $$
% The content loss can be formulated as
% $
% L_{content} = \lambda_{ssim}L_{ssim} + \lambda_{mae}L_{mae}
% $.


% The semantic loss consists of two parts: $L_{level}$ and
% $L_{cmp}$.
% The $L_{level}$ is focal loss \cite{lin2017focal} and the $L_{cmp}$ is the cosine similarity loss between the feature of $I_{IHC}$ and  $\hat{I}_{IHC}$ extracted by the comparator $C$.
% The semantic loss can be formulated as
% $
% L_{semantic} = \lambda_{level}L_{level}+\lambda_{cmp}L_{cmp}
% $.

% For adversarial learning, we use the multi-scale patch GAN loss \cite{pix2pixhd} for adversarial learning, which can be formulated as

% $
% L_{G A N} =\frac{1}{2}\times(\arg \min _G \max _D\left(L_{G A N}^{512}\left(\hat{I}_{IHC}, I_{IHC}\right)\right. \left.+L_{G A N}^{256}\left(\hat{I}_{IHC}, I_{IHC}\right)\right) )
% $
% The $L_{GAN}^{256}$ is computed the same way as $L_{GAN}^{512}$ but uses resized $I_{IHC}$ and $\hat{I}_{IHC}$.

% \noindent \textbf{Overall Loss.}
% The overall loss is formulated as follows:
% $$
% L= \lambda_{Stain}L_{Stain}+\lambda_{content}L_{content}+\lambda_{semantic}L_{semantic}+\lambda_{GAN}L_{GAN} 
% $$
\subsection{Loss Functions}
\noindent \textbf{Overall Loss.}
The overall loss function is formulated as follows:
\begin{equation}
L= \lambda_{stain}L_{stain}+\lambda_{content}L_{content}+\lambda_{level}L_{level}+\lambda_{GAN}L_{GAN}, 
\end{equation}
which contains $L_{stain}$ and auxiliary loss including $L_{content}, L_{level},$ and $L_{GAN}$.

\noindent \textbf{Stain Loss. } The stain loss is the most significant loss in our framework, which is the weighted sum of $ L_{{H}}$ and $ L_{{DAB}}$, whose purpose and formulation have been discussed in the former section respectively. 
The stain loss is formulated as:
\begin{equation}
L_{stain} = \lambda_{H}L_{H}+\lambda_{DAB}L_{DAB}.
\end{equation}
\textbf{Auxiliary Losses. }Besides the stain loss, we also incorporates auxiliary losses to facilitate the generation of IHC images.
The content loss comprises structural similarity loss $L_{ssim}$ \cite{ssim} , mean absolute error loss $L_{mae}$, and comparator loss $L_{cmp}$. $L_{ssim}$ and $L_{mae}$ are calculated directly between $\hat{I}_{IHC}$ and $I_{IHC}$, while $L_{cmp}$ represents the cosine similarity loss between features of $\hat{I}_{IHC}$ and $I_{IHC}$, as extracted by comparator C.
The content loss can be formulated as
$
L_{content} = \lambda_{ssim}L_{ssim} + \lambda_{mae}L_{mae} + \lambda_{cmp}L_{cmp}
$.
The HER2 level loss $L_{level}$ is a focal loss applied to $f_{level}$ to obtain more precise HER2-level information for the feature fusion module.
For the GAN loss $L_{GAN}$, the multi-scale patch GAN loss is employed as the loss function, which is the mean value of the patch GAN loss in resolution of 512 and 256.



==> parts/Methods.tex <==
\section{Methods}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/modelfig.png}
    \caption{The overall architecture of our framework. H\&E images are inputted into the Destainer for removal of the Eosin channel and subsequently brought into closer alignment with the Hematoxylin channel of IHC images in the high-dimensional feature space. The high-level representation of $H\&E_{H}$ and the level information of HER2  are directed into the Feature Fusion module. The Restainer generates the corresponding IHC images. E is a down-sampler, C and D are comparator and discriminator respectively  }
    \label{model}
\end{figure}

\subsection{Staining Separation}
To achieve stain separation, we map a tissue pathology image in the RGB space to the HED space (Hematoxylin, Eosin, Diaminobenzidine) through a linear transformation, obtaining an image in the HED space. Stain elimination is then accomplished by setting two channels of this HED space image to zero.
For example,if we aim to preserve the a certain channel of a particular stained image. We denoted this image as $M$, the projection matrix to HED space as $P^{\dagger}$, in which $P^{\dagger}$ is the Moore-Penrose Inverse of P. The stain separation result can be formulated as
$$M_{res}= \exp{((\log M) P^{\dagger}QP)}$$
, The space projection matrices $P$ and $Q$ for channel isolation are defined as
\[
P = \begin{bmatrix}
0.65 & 0.70 & 0.29 \\
0.07 & 0.99 & 0.11 \\
0.27 & 0.57 & 0.78
\end{bmatrix} \quad
Q = \begin{bmatrix}
\delta(1, c) & 0 & 0 \\
0 & \delta(2, c) & 0 \\
0 & 0 & \delta(3, c)
\end{bmatrix}
\]
where $\delta(i, c)$ be a function defined as
\[
\delta(i, c) = \begin{cases} 
1, & \text{if } i = c \\
0, & \text{otherwise}
\end{cases}
\]
where $i \in \{1, 2, 3\}$ corresponds to the matrix index and $c \in \{1, 2, 3\}$ corresponds to the channel we wish to retain (1 for Hematoxylin, 2 for Eosin, 3 for Diaminobenzidine), the values in the matrix that contain the information of others two channels are set to 0.
\subsection{DeReStainer}
The architecture of our framework is shown in \autoref{model}. The generator of the architecture is modified from the typical resnet-9 block generator. Our framework initially employs a staining separation algorithm to filter out the Eosin channel from the input H\&E images. Subsequently, based on the predicted HER2 level information, the images are stained to the corresponding IHC image. The entire staining principle aligns with medical reasoning.
\subsubsection{Training Algorithm}
Our framework employs fully supervised training. The Destainer in our framework contains a staining separation model and an encoder. During the training process, the staining separation algorithm is applied simultaneously to both the H\&E images $I_{H\&E}$ and their corresponding IHC images $I_{IHC}$. The separated Hematoxylin channel images from both, which are denoted as $I_{H\&E,H}$ and $I_{IHC,H}$ are then fed into the encoder of Destainer. After passing through the Destainer, both sets of images are concurrently inputted into $E_{Hema}$, which brings closer the $I_{H\&E,H}$ and $I_{IHC,H}$. Additionally, $I_{H\&E,H}$ is directed into $E_{level}$, which concludes with a linear layer for the prediction of HER2 level, utilizing focal loss \cite{lin2017focal} as the loss function. The classification information encoded by $E_{level}$, along with the Hematoxylin channel features of the H\&E images encoded by the Destainer, are jointly directed into the Feature Fusion module.

The feature fusion module consists of 9 basic blocks, denote the input of a basic block as $x$ then each of them can be formulated as
$$
y = Att(ActMod^2(x,E_{level}(x)))+x
$$
In which $Att$ is the SimAM\cite{simam}, a parameter-free attention layer. $ActMod$ is the composition of the LeakyRelu activation function and a weight demodulation operation \cite{stylegan}. The demodulation operation can be formulated as
$$
x^{’} = \text{Conv2d}\left( x, \frac{W \times (E_{level}(x) + 1)}{\sqrt{\sum(W \times (E_{level}(x) + 1))^2 + \epsilon}} \right) + b
$$, where $W$ is the original weight of the convolutional layer, $b$ is an optional bias, and $\epsilon$ is a small constant, which is $1e-8$ in our setting.
\subsection{Loss Functions}
In our framework, several loss functions were applied to constrain the image content as well as the semantic information of the generated IHC image. This section describes the losses including content loss, semantic loss, GAN loss and De-Re staining loss in detail. For the sake of simplicity, we denote $I_{IHC}$ as the ground truth IHC image for the input $H\&E$ image and $\hat{I_{IHC}}$ as the generated IHC image of our framework.

\subsubsection{Content Loss}
The content loss consists of $L_{ssim}$ (structure similarity loss) and the $L_{mae}$ mean absolute error loss. 
$$L_{mae} = \|\hat{I_{IHC}}-I_{IHC}\|_1,L_{ssim}=1-SSIM(\hat{I_{IHC}}-I_{IHC})
$$
the content loss can be formulated as:
$$
L_{content} = \lambda_{mae}L_{mae}+\lambda_{ssim}L_{ssim}
$$

\subsubsection{Semantic Loss}
The semantic loss consists of two parts: $L_{level}$ and
$L_{cmp}$.
The $L_{level}$ is focal loss \cite{lin2017focal} and the $L_{cmp}$ is the cosine similarity loss between the feature of $I_{IHC}$ and  $\hat{I_{IHC}}$ extracted by the comparator $C$. The comparator $C$ is a resnet-50 backbone trained on the training set of BCI dataset using the HER2 level label. 
The semantic loss can be formulated as:
$$
L_{semantic} = \lambda_{level}L_{level}+\lambda_{cmp}L_{cmp}
$$
\subsubsection{GAN Loss}
The discriminator we use is the multi-scale discriminator in Pix2PixHD\cite{pix2pixhd}. The loss function can be formulated as:
$$
\begin{aligned}
L_{G A N} & =\frac{1}{2}\times(\arg \min _G \max _D\left(L_{G A N}^{512}\left(\hat{I}_{i h c}, I_{IHC}\right)\right. \left.+L_{G A N}^{256}\left(\hat{I}_{IHC}, I_{i h c}\right)\right) )
\end{aligned}
$$
The $L_{GAN}^{256}$ is computed in the same way as $L_{GAN}^{512}$ but uses resized $I_{IHC}$ and $\hat{I_{IHC}}$.
\subsubsection{Stain Loss}
The Staining loss is a loss function proposed in conjunction with a stain separation algorithm, designed to regulate the effects of de-staining and re-staining. This loss function comprises two components: Hematoxylin loss \( L_{\text{Hematoxylin}} \) and DAB loss \( L_{\text{DAB}} \). The Hematoxylin loss is utilized to align the high-level representations of the Hematoxylin channel in H\&E staining with the Hematoxylin channel IHC in the encoder, using a cosine similarity loss. Meanwhile, the DAB loss involves applying MAE loss to the DAB channel of both the generated IHC image and the ground truth. This approach aims to enhance the quality of the staining. The $L_{\text{Hematoxylin}}$ and $L_{\text{DAB}}$ can be formulated as 
$$
L_{\text{Hematoxylin}} = 1-\frac{E_{hemato}(Destainer(I_{H\&E,H}))\cdot E_{hemato}(Destainer(I_{IHC,H}))}{\|E_{hemato}(Destainer(I_{H\&E,H})\| \cdot \| E_{hemato}(Destainer(I_{IHC,H})\|}
$$
$$
L_{\text{DAB}} = \|\hat{I_{IHC,DAB}}-I_{IHC,DAB}\|_1
$$
the stain loss can be formulated as:
$$
L_{Stain} = \lambda_{Hematoxylin}L_{Hematoxylin}+\lambda_{DAB}L_{DAB}
$$
\subsubsection{Overall Loss}
The overall loss can be formulated as:
$$
L= \lambda_{content}L_{content}+\lambda_{semantic}L_{semantic}+\lambda_{GAN}L_{GAN} + \lambda_{Stain}L_{Stain}
$$


==> parts/lit.tex <==
\section{Literature Review}
There are many benchmark frameworks for this task in deep learning. 
For unsupervised methods, CycleGAN \cite{zhu2017unpaired} uses a novel cycle-consistency loss for domain translation without paired examples.
This innovative approach employs dual GAN structures, each responsible for one direction of domain translation, and enforces a cycle-consistency to ensure that the original image can be reconstructed from the translated image, thereby aligning the distribution of translated images with the target domain without the need for paired training samples. 
However, for many tasks, the lack of supervision from labeled data will cause the strict decrease of model's accuracy. 
To overcome unsupervised methods' accuracy drop, introducing a supervised I2IT framework is essential. 
Pix2Pix\cite{pix2pix} employed a cGAN for effective image translation in paired datasets. Building upon this foundation. Pix2PixHD \cite{pix2pixhd} enhanced the resolution of generated images with a multi-scale architecture. In medical image analysis, specialized models have been developed to address the H\&E to IHC translation, emphasizing the complexity and clinical relevance of pathological images. Liu et al. launched the Breast Cancer Immunohistochemical (BCI) competition and introduced the Pyramid Pix2Pix model which imposed stricter constrain on structural similarity for the staining translation task in H\&E images \cite{liu2022bci}. Li et al. applied PatchNCE loss to mitigate dataset alignment issues in BCI dataset \cite{li2023adaptive}. Despite achieving commendable results on structural metrics such as the Structural Similarity Index (SSIM) and the Peak Signal-to-Noise Ratio (PSNR) which are pivotal for assessing images' intrinsic properties, we observed that the IHC images produced by previous methods sometimes do not fully reflect the HER2 level information of the ground truth IHC images. This can lead to a less precise representation of the HER2 level in the pathology tissue, which may affect clinical significance.

==> parts/loss_function.tex <==
\newpage
\subsection{Loss Functions}
\noindent \textbf{Overall Loss.}
The overall loss function is formulated as follows:
$$
L= \lambda_{Stain}L_{Stain}+\lambda_{content}L_{content}+\lambda_{level}L_{level}+\lambda_{GAN}L_{GAN}, 
$$
which contains stain loss and auxiliary loss including content loss, HER2 level loss and GAN loss.

\noindent \textbf{Stain Loss. } The stain loss is the most significant loss in our framework, which is the weighted sum of $ L_{{H}}$ and $ L_{{DAB}}$, whose purpose and formulation have been discussed in the former section respectively. 
The stain loss is formulated as:
$$
L_{stain} = \lambda_{H}L_{H}+\lambda_{DAB}L_{DAB}.
$$
\textbf{Auxiliary Losses. }Besides the stain loss, we also incorporates auxiliary losses to facilitate the generation of IHC images.

The content loss comprises structural similarity loss $L_{ssim}$ \cite{ssim}, mean absolute error loss $L_{mae}$, and comparator loss $L_{cmp}$. $L_{ssim}$ and $L_{mae}$ are calculated directly between $\hat{I}_{IHC}$ and $I_{IHC}$, while $L_{cmp}$ represents the cosine similarity loss between features of $\hat{I}_{IHC}$ and $I_{IHC}$, as extracted by comparator C.
The content loss can be formulated as
$
L_{content} = \lambda_{ssim}L_{ssim} + \lambda_{mae}L_{mae} + \lambda_{cmp}L_{cmp}
$.

The HER2 level loss $L_{level}$ is a focal loss\cite{lin2017focal} applied to $f_{level}$ to obtain more precise HER2-level information for the feature fusion module.

For the GAN loss $L_{GAN}$, the multi-scale patch GAN loss \cite{pix2pixhd} is employed as the loss function, which is the mean value of the patch GAN loss \cite{pix2pix} in resolution of 512 and 256.


